PPT-GNN: A Practical Pre-Trained Spatio-Temporal Graph Neural Network for Network Security

Recent works have demonstrated the potential of Graph Neural Networks (GNN) for network intrusion detection. Despite their advantages, a significant gap persists between real-world scenarios, where detection speed is critical, and existing proposals, which operate on large graphs representing several hours of traffic. This gap results in unrealistic operational conditions and impractical detection delays. Moreover, existing models do not generalize well across different networks, hampering their deployment in production environments. To address these issues, we introduce PPTGNN, a practical spatio-temporal GNN for intrusion detection. PPTGNN enables near real-time predictions, while better capturing the spatio-temporal dynamics of network attacks. PPTGNN employs self-supervised pre-training for improved performance and reduced dependency on labeled data. We evaluate PPTGNN on three public datasets and show that it significantly outperforms state-of-the-art models, such as E-ResGAT and E-GraphSAGE, with an average accuracy improvement of 10.38%. Finally, we show that a pre-trained PPTGNN can easily be fine-tuned to unseen networks with minimal labeled examples. This highlights the potential of PPTGNN as a general, large-scale pre-trained model that can effectively operate in diverse network environments.

==> features.tex <==
\begin{table}[hb]
\label{tab:my-table}
\tiny
 \resizebox{\textwidth}{!}{
\begin{tabular}{|llc|}
\hline
\textbf{Column name}                   & \textbf{Feature}                                                                                                              & \textbf{Value}       \\ \hline
src\_ip                                & Source IP address                                                                                                             & Str                  \\
src\_port                              & Source Port                                                                                                                   & Int                  \\
dst\_ip                                & Destination IP address                                                                                                        & Str                  \\
protocol                               & Destination port                                                                                                              & Int                  \\
ip\_version                            & IP version                                                                                                                    & Int                  \\
bidirectional\_first\_seen\_ms         & Timestamp in milliseconds of the first seen packet of the flow                                                                & Int                  \\
bidirectional\_last\_seen\_ms          & Timestamp in milliseconds of the last seen packet of the flow                                                                 & Int                  \\
bidirectional\_duration\_ms            & Duration of the entire flow in milliseconds                                                                                   & Int                  \\
bidirectional\_packets                 & Total packets of the flow                                                                                                     & Int                  \\
bidirectional\_bytes                   & Total bytes of the flow                                                                                                       & Int                  \\
bidirectional\_min\_packet\_size       & Minimum packet size of the flow                                                                                               & Int                  \\
bidirectional\_max\_packet\_size       & Maximum packet size of the flow                                                                                               & Int                  \\
bidirectional\_mean\_packet\_size      & Mean of the size of the packet flows                                                                                          & Float                \\
bidirectional\_mean\_packet\_iat\_ms   & Mean of the inter arrival packet time of all the packets of the flow in milliseconds                                          & Float                \\
bidirectional\_cumulative\_flags       & Logical OR of the flags of all the packets of the flow                                                                        & Int                  \\
src2dst\_first\_seen\_ms               & Timestamp in milliseconds of the first seen packet from source to destination IP address                                      & Int                  \\
src2dst\_last\_seen\_ms                & Timestamp in milliseconds of the last seen packet from source to destination IP address                                       & Int                  \\
src2dst\_duration\_ms                  & Total duration of the source to destination packets in milliseconds                                                           & Int                  \\
src2dst\_packets                       & Total packets sent from source to destination IP address                                                                      & Int                  \\
src2dst\_bytes                         & Total bytes sent from source to destination IP address                                                                        & Int                  \\
src2dst\_min\_packet\_size             & Minimum packet size sent from source to destination IP address                                                                & Int                  \\
src2dst\_max\_packet\_size             & Maximum packet size sent from source to destination IP address                                                                & Int                  \\
src2dst\_mean\_packet\_size            & Mean of the size of the packets sent from source to destination IP address                                                    & Float                \\
src2dst\_mean\_packet\_iat\_ms         & Mean of the inter arrival packet time of all the packets sent from source to destination IP address in milliseconds           & Float                \\
src2dst\_cumulative\_flags             & Logical OR of the flags of all the packets sent from source to destination IP address                                         & Int                  \\
dst2src\_first\_seen\_ms               & Timestamp in milliseconds of the first seen packet from destination to source IP address                                      & Int                  \\
dst2src\_last\_seen\_ms                & Timestamp in milliseconds of the last seen packet from destination to source IP address                                       & Int                  \\
dst2src\_duration\_ms                  & Total duration of the destination to source packets in milliseconds                                                           & Int                  \\
dst2src\_packets                       & Total packets sent from destination to source IP address                                                                      & Int                  \\
dst2src\_bytes                         & Total bytes sent from destination to source IP address                                                                        & Int                  \\
dst2src\_min\_packet\_size             & Minimum packet size sent from destination to source IP address                                                                & Int                  \\
dst2src\_max\_packet\_size             & Maximum packet size sent from destination to source IP address                                                                & Int                  \\
dst2src\_mean\_packet\_size            & Mean of the size of the packets sent from destination to source IP address                                                    & Float                \\
dst2src\_mean\_packet\_iat\_ms         & Mean of the inter arrival packet time of all the packets sent from destination to source IP address in milliseconds           & Float                \\
dst2src\_cumulative\_flags             & Logical OR of the flags of all the packets sent from destination to source IP address                                         & Int                  \\
classification                         & Labeling of the dataset (0 or 1)                                                                                              & Int                  \\
category                               & Category of the classification if present                                                                                     & Str                  \\
subcategory                            & Subcategory of the classification if present                                                                                  & Str                  \\ \hline
\end{tabular}}
\end{table}
